Competent but Rigid: Identifying the Gap in Empowering AI to Participate Equally in Group Decision-Making

Existing research on human-AI collaborative decision-making focuses mainly on the interaction between AI and individual decision-makers. There is a limited understanding of how AI may perform in group decision-making. This paper presents a wizard-of-oz study in which two participants and an AI form a committee to rank three English essays. One novelty of our study is that we adopt a speculative design by endowing AI equal power to humans in group decision-making.We enable the AI to discuss and vote equally with other human members. We find that although the voice of AI is considered valuable, AI still plays a secondary role in the group because it cannot fully follow the dynamics of the discussion and make progressive contributions. Moreover, the divergent opinions of our participants regarding an "equal AI" shed light on the possible future of human-AI relations.

==> tables/model_performance.tex <==
\begin{table}[htbp]
 \centering
 \begin{tabular}{lccccc}\toprule
    & Content & Organization & Style & Conventions & Overall \\\midrule
    Taghipour and Ng~\cite{taghipour2016neural} & - & - & - & - &  0.811 \\
    Kumar et al.~\cite{kumar-etal-2022-many} & - & - & - & - & 0.795 \\
    Ours   & 0.780 & 0.713 & 0.766 & 0.748 & 0.815   \\\bottomrule
 \end{tabular}
 \caption{The performance of our ML model on \textit{essay set 7}, evaluated by Cohen’s Kappa with quadratic weights.}
 \label{tab:model_performance}
\end{table}
